Fixed parameter complexity of distance constrained labeling and uniform channel assignment problems

We study computational complexity of the class of distance-constrained graph labeling problems from the fixed parameter tractability point of view. The parameters studied are neighborhood diversity and clique width. We rephrase the distance constrained graph labeling problem as a specific uniform variant of the Channel Assignment problem and show that this problem is fixed parameter tractable when parameterized by the neighborhood diversity together with the largest weight. Consequently, every $L(p_1, p_2, \dots, p_k)$-labeling problem is FPT when parameterized by the neighborhood diversity, the maximum $p_i$ and $k.$ Our results yield also FPT algorithms for all $L(p_1, p_2, \dots, p_k)$-labeling problems when parameterized by the size of a minimum vertex cover, answering an open question of Fiala et al.: Parameterized complexity of coloring problems: Treewidth versus vertex cover. The same consequence applies on Channel Assignment when the maximum weight is additionally included among the parameters. Finally, we show that the uniform variant of the Channel Assignment problem becomes NP-complete when generalized to graphs of bounded clique width.

==> src/results.tex <==
\section{The {\sc Channel Assignment} parameterized by vertex-cover}\label{s:metaalg}

We now use the results of the previous sections to derive an \FPT\ algorithm proposed as Theorem~\ref{thm:chaVC}. Further on, we will discuss in general, how to derive similar results based on the relation between vertex cover and neighborhood diversity parameters.

\begin{proof}[Proof of Theorem~\ref{thm:chaVC}]
Recall that for a graph $G$ it holds that $\nd(G)\le2^{\vc(G)} + \vc(G)$ since it is possible to construct the type graph $T$ of $G$ as follows. Let $U$ be the optimal vertex cover of $G.$ For each vertex $u\in U,$ we introduce a vertex to the type graph (call this vertex $u$ again). Next let $I = V(G)\setminus U$ be the independent set of $G.$ We subdivide $I$ into sets for every subset $X\subseteq U$:
$$I_X := \{v\in I\colon \{v,x\}\in E(G) \text{ for } x\in X \text{ and } \{v,x\}\notin E(G) \text{ for } x\notin X\}.$$
Now it is easy to see that the sets defined form a neighborhood diversity decomposition and that the size of the decomposition is at most $2^{\vc(G)} + \vc(G).$

\begin{figure}[ht!]
  \input{tikz/decompositionRefinement.tikz}
  \caption{An example of a neighborhood diversity decomposition based on vertex cover---sets $I_X$ in the bottom.}
\end{figure}

Before we apply Theorem~\ref{thm:cha}, we have refine sets $I_X$ further more, so that the edge-weights are uniform. For a set $X = \{x_1,\dots,x_k\}\subseteq U$ and a tuple of positive integers $\bw = (w_1,\dots,w_k)$ with $0<w_i\le w_{\max}$ for every $1\le i\le k$ we define the set $I_X^\bw$ as
$$I_X^\bw := \{v\in I_X\colon w(v,x_i) = w_i\text{ for } 1\le i\le k\}.$$

Observe that a refinement of a neighborhood diversity decomposition is again a decomposition. We now estimate the number of types of the refined decomposition. The number of types of the refined decomposition can be upper-bounded by $\vc(G) + (2^{\vc(G)})w_{\max}^{\vc(G)}.$ We can now apply Theorem~\ref{thm:cha} on the refined decomposition. This finishes the proof.
\end{proof}

%\paragraph*{Proof comment}
This proof might be interesting on its own as it yields a general method for finding an \FPT{} algorithm for an edge-constrained problem parameterized by the size of vertex cover via its {\em uniform version} parameterized by the neighborhood diversity. 

If a problem {\sc P} with edge-constraints allows the existence of an
equivalence relation $R$ on the set of edges, a bound $b_G$ and a function
$r:\N\times\N\rightarrow\N,$ such that the number of equivalence
classes of an independent set is at most $r(\vc(G), b_G)$, and
furthermore, if a problem {\sc Uniform P} admits an \FPT algorithm
when parameterized by neighborhood diversity, then the original problem {\sc P}
admits an \FPT algorithm when parameterized by $\vc$ and $b$.

Moreover, if there exists a function $q:\N\rightarrow\N$ such that $r(\vc(G), b_G) \le q(\vc(G)),$ then problem {\sc P} becomes \FPT when parameterized by the size of vertex cover only.


